AutoBlock: A Hands-off Blocking Framework for Entity Matching

Entity matching seeks to identify data records over one or multiple data sources that refer to the same real-world entity. Virtually every entity matching task on large datasets requires blocking, a step that reduces the number of record pairs to be matched. However, most of the traditional blocking methods are learning-free and key-based, and their successes are largely built on laborious human effort in cleaning data and designing blocking keys. In this paper, we propose AutoBlock, a novel hands-off blocking framework for entity matching, based on similarity-preserving representation learning and nearest neighbor search. Our contributions include: (a) Automation: AutoBlock frees users from laborious data cleaning and blocking key tuning. (b) Scalability: AutoBlock has a sub-quadratic total time complexity and can be easily deployed for millions of records. (c) Effectiveness: AutoBlock outperforms a wide range of competitive baselines on multiple large-scale, real-world datasets, especially when datasets are dirty and/or unstructured.

==> figures/LSH.tex <==
\begin{tikzpicture}[
%   scale=0.9,
	axis/.style={very thick, -latex},
	embedding/.style={draw, thick, minimum width=1*2ex, minimum height=6*2ex, inner sep=0},
	label/.style={rectangle, thick, minimum height=20, minimum width=70, node font=\bf\Large},
	dot/.style={circle, inner sep=2.5, draw, thick, fill=white}
	]

	\draw[axis] (-0.3, 0) -- (4, 0);
	\draw[axis] (0, -0.3) -- (0, 4);

	\fill[Lavender] (1.3, 3) ellipse[x radius=1, y radius=0.8];
	\fill[ProcessBlue] (1.5, 1) ellipse[x radius=0.5, y radius=0.8];
	\fill[LimeGreen] (3, 2) ellipse[x radius=0.7, y radius=0.8];

	\node[label, draw] (B1) at (6, 3.5) {Bucket 1};
	\node[label, fill=Gray, draw, below=0 of B1.south] (B2) {Bucket 2};
	\node[label, draw, below=0 of B2.south] (B3) {Bucket 3};
	\node[label, fill=Gray, draw, below=0 of B3.south] (B4) {Bucket 4};
	\node[label, draw, below=0 of B4.south] (B5) {Bucket 5};

	\draw[latex-] (B1.west) -- (0.9, 2.8) node[dot] {};
	\draw[latex-] (B1.west) to[bend left=-5] (1.2, 3.3) node[dot] {};
	\draw[latex-] (B1.west) to[bend left=5] (1.5, 2.7) node[dot] {};

	\draw[latex-] (B5.west) to[bend left=-5] (1.5, 1.4) node[dot] {};
	\draw[latex-] (B5.west) -- (1.4, 1)   node[dot] {};
	\draw[latex-] (B5.west) to[bend left=5] (1.6, 0.7) node[dot] {};

	\draw[latex-] (B3.west) to[bend left=5] (3, 1.7)   node[dot] {};
	\draw[latex-] (B3.west) -- (2.8, 2)   node[dot] {};
	\draw[latex-] (B3.west) to[bend left=-5] (2.9, 2.3) node[dot] {};

\end{tikzpicture}

==> figures/performance_scatterplot.tex <==
\begin{tikzpicture}[
    axis/.style={very thick, ->, -latex},
    dashed line/.style={densely dotted, thin},
    dot/.style={circle, minimum size=3ex, inner sep=0, fill=orange},
    label/.style={align=center, node font=\large \bfseries},
    axis_label/.style={align=center, node font=\LARGE \bfseries},
    ]
    
	\draw[axis] (-0.2, 0) -- (8.2, 0) node[axis_label, midway, below=2ex] {Human Effort};
  	\draw[axis] (0, -0.2) -- (0, 4.2) node[axis_label, midway, rotate=90, above=1ex] {Recall};
  	
    \draw[dashed line] (1.2, 0) node[label, below]{hour} -- (1.2, 4.2);
    \draw[dashed line] (4, 0) node[label, below]{day} -- (4, 4.2);
    \draw[dashed line] (6.8, 0) node[label, below]{week} -- (6.8, 4.2);
    
    \coordinate[dot, fill=cPurple](a) at (1, 1.1) node[label, below=0 of a] {Single Key}; 
    \coordinate[dot, fill=cGreen](b) at (1.5, 2.4) node[label, below=0 of b] {Disjunctive Key \\ \cite{Bilenko2006,Michelson2006}};   
    \coordinate[dot, fill=cBlue](c) at (3.8, 3.3) node[label, below=0 of c]{MinHash \cite{Liang2014}}; 
    \coordinate[dot, fill=cGold](d) at (6.8, 3.6) node[label, below=0 of d]{Customized Key \\ \cite{Gravano2003,Aizawa2005,Papadakis2013} };
    \coordinate[dot, fill=cRed](e) at (2.0, 4.0) node[label, below=0 of e]{\method};
     
\end{tikzpicture}

==> tables/notation.tex <==
\small
\begin{tabular}{ll}
	\toprule
	\textbf{Notation}                                       & \textbf{Meaning}                                          \\
	$n$                                                     & \# of tuples                                              \\
	$m$                                                     & \# of attributes                                          \\
	$\x_i$                                                  & $i$-th tuple                                              \\
	$\X \defas [\x_1, \ldots, \x_n]$                        & Tuple set                                                 \\
	$\a_{ij}$                                               & $j$-th attribute of $i$-th tuple                          \\
	$w_{ijk}$                                               & $k$-th token of $j$-th attribute of $i$-th tuple          \\
	$l_{ij}$                                                & the length of $j$-th attribute of $i$-th tuple            \\
	$\cA_j$                                                 & Domain of $j$-th  attribute                               \\
	$\cV_j$                                                 & Vocabulary for $j$-th attribute.                          \\
	$\x_i \defas \{\a_{ij}\}_{j = 1}^m$                     & $i$-th tuple consists of $m$ attributes                   \\
	$\a_{ij} \defas \{w_{ijk}\}_{k = 1}^{l_{ij}}$           & $j$-th attr. of $i$-th tuple consists of $l_{ij}$ tokens. \\
	$\v_w$                                                  & token embedding for word $w$                              \\
	$\sigma(\cdot, \cdot)$                                  & Similarity function                                       \\
	$g_j(\v_1, \v_2, \ldots)$                               & $j$-th attribute encoder                                  \\
	$\g^{(j)}_i \defas g_j(\a_{ij})$                        & attribute embedding for attribute $\a_{ij}$               \\
	$f_s(\g_1, ,\cdots, \g_m)$                              & signature function                                        \\
	$\f^{(s)}_i \defas f_s(\g^{(i)}_1, \ldots, \g^{(i)}_m)$ & $s$-th signature vector for tuple $\x_i$.                 \\
	$S$                                                     & number of signature functions.                            \\
	$\cL \defas \{(i,i')\}$                                 & A set of weakly matched pairs.                            \\
	$\cT \defas \{(i,i')\}$                                 & The set of true matched pairs.                            \\
	$\cC \defas \{(i,i')\}$                                 & The set of candidate pairs.                               \\
	$\theta$                                                & similarity threshold                                      \\
	$B$                                                     & LSH tables                                                \\
	$K$                                                     & bits/LSH functions per table                              \\ \bottomrule
\end{tabular}


==> tables/salesman.tex <==
\begin{tabular}{ c|c|c|c|c||c|}
	Feature       & \rotatebox{70}{Single-key} & \rotatebox{70}{Multi-key} & \rotatebox{70}{Customized-key} & \rotatebox{70}{MinHash \cite{liang2014noise}} & \rotatebox{70}{\method} \\ \midrule
	High recall   &                            &                           &         \CheckmarkBold         &                \CheckmarkBold                 &     \CheckmarkBold      \\
	Low P/E ratio &       \CheckmarkBold       &      \CheckmarkBold       &                                &                                               &     \CheckmarkBold      \\
	Efficiency    &       \CheckmarkBold       &      \CheckmarkBold       &         \CheckmarkBold         &                \CheckmarkBold                 &     \CheckmarkBold      \\
	Hands-off     &       \CheckmarkBold       &                           &                                &                                               &     \CheckmarkBold      \\ \bottomrule
\end{tabular} 
